On the workflow, opportunities and challenges of developing foundation model in geophysics

Foundation models, as a mainstream technology in artificial intelligence, have demonstrated immense potential across various domains in recent years, particularly in handling complex tasks and multimodal data. In the field of geophysics, although the application of foundation models is gradually expanding, there is currently a lack of comprehensive reviews discussing the full workflow of integrating foundation models with geophysical data. To address this gap, this paper presents a complete framework that systematically explores the entire process of developing foundation models in conjunction with geophysical data. From data collection and preprocessing to model architecture selection, pre-training strategies, and model deployment, we provide a detailed analysis of the key techniques and methodologies at each stage. In particular, considering the diversity, complexity, and physical consistency constraints of geophysical data, we discuss targeted solutions to address these challenges. Furthermore, we discuss how to leverage the transfer learning capabilities of foundation models to reduce reliance on labeled data, enhance computational efficiency, and incorporate physical constraints into model training, thereby improving physical consistency and interpretability. Through a comprehensive summary and analysis of the current technological landscape, this paper not only fills the gap in the geophysics domain regarding a full-process review of foundation models but also offers valuable practical guidance for their application in geophysical data analysis, driving innovation and advancement in the field.

==> contributions.tex <==
\paragraph{Author Contributions}
Percy Liang initiated and conceptualized the framing and structure of the overall report. 
He and Rishi Bommasani worked together to lead the decentralized writing effort and provided guidance on individual sections. 
Drew A. Hudson created all the figures in the report, discussing their structure and content with the authors of each section. 
Each of the 26 sections of this report was written by a subset of authors, whose names are listed at the beginning of each section. 
There were, however, many discussions that spanned multiple sections, so the actual contributions to each section generally came from a broader set. 
Finally, we note that not all the views expressed in this report are held by all the authors.

==> origins.tex <==
In March 2021, we created an informal community at Stanford University of students, faculty, and researchers
interested in some aspect of foundation models.\footnote{This community
led to the founding of the \emph{Center for Research on Foundation Models (CRFM)},
a new interdisciplinary initiative at the Stanford Institute for Human-Centered AI (HAI).}
From the very beginning, the community included not just AI researchers,
but those eager to apply foundation models to their domain (\eg{}healthcare and law),
as well as those who were interested in societal concerns (\eg{}ethics and economics).
As discussions progressed,
we noticed that there were many gaps in mutual understanding\dash{}how the
technology worked, how industry develops foundation models, how to think about the ethical
concerns, etc.,
and existing literature only covered bits and pieces.
We wanted to therefore provide a fuller picture of foundation models, identify
opportunities and risks, and establish a constructive vision for the future responsible development of foundation models.

The writing of this report was an experiment:
we had over 100 people from different backgrounds come together to write a
single report covering a wide range of aspects of foundation models.
A large part of this report is a survey of existing work, but through many discussions,
we have unified it in one report to highlight all the interdisciplinary connections.
